SemTalk: Holistic Co-speech Motion Generation with Frame-level Semantic Emphasis

Co-speech gesture generation must carefully integrate common rhythmic motion with rare yet essential semantic gestures. In this work, we propose SemTalk for holistic co-speech gesture generation with frame-level semantic emphasis. Our key insight is to separately learn base motions and sparse motions, and then adaptively fuse them. In particular, coarse2fine cross-attention module and rhythmic consistency learning are explored to establish rhythm-related base motion, ensuring a coherent foundation that synchronizes gestures with the speech rhythm. Subsequently, semantic emphasis learning is designed to generate semantic-aware sparse motion, focusing on frame-level semantic cues. Finally, to integrate sparse motion into the base motion and generate semantic-emphasized co-speech gestures, we further leverage a learned semantic score for adaptive synthesis. Qualitative and quantitative comparisons on two public datasets demonstrate that our method outperforms the state-of-the-art, delivering high-quality co-speech motion with enhanced semantic richness over a stable base motion.

==> sec/2_related_2.tex <==
\section{Related Work}

\textbf{Co-speech Gesture Generation.} The evolution of co-speech gesture generation reflects a shift from rule-based methods [8, 18, 22, 38, 44] to complex, data-driven models aimed at capturing the nuanced relationship between speech and gestures. Initial deterministic approaches—using models such as MLPs [24], CNNs [14], and RNNs [5, 15, 27]—attempted to directly map speech features to gestures but struggled to capture the variability of natural motion. To address these limitations, recent methods have increasingly adopted probabilistic models, such as normalizing flows [48], GANs [14], and diffusion models [1, 47, 54], which provide enhanced flexibility and realism. For example, diffusion-based models like DiffGesture [54] and DiffuseStyleGesture [47] are capable of generating diverse gesture patterns, though they rely on initial gesture inputs, limiting spontaneous generation across longer sequences.

Parallel advancements have explored the integration of semantic information to increase the contextual relevance of gestures. For instance, models such as Speech2AffectiveGesture [7] and HA2G [40] use audio and textual conditioning to align gestures more closely with the semantic content of speech, while SEEG [37] employs VQ-VAE to classify gestures for semantic consistency. LivelySpeaker introduces a two-stage framework to synchronize and contextualize gestures. However, by processing semantic and rhythmic gestures in separate stages, LivelySpeaker may struggle to maintain fine-grained integration between rhythm and semantics, particularly in dynamic or real-time interactions. Additionally, this reliance on a sequential process can limit adaptability when spontaneous or sparsely needed semantic gestures are required. To address these gaps, our proposed CHARM model integrates rhythmic and semantic relevance within a single framework. Through rhythmic consistency loss, CHARM ensures a coherent base motion, while a semantic gating mechanism activates contextually significant gestures at the frame level, achieving rhythmically natural and semantically meaningful gestures without dependence on rigid templates.

\textbf{Co-speech Holistic Motion Generation.} Generating expressive, synchronized full-body motion in response to speech poses significant challenges, particularly in achieving coherence across regions such as the face, hands, and torso, which are critical for naturalistic co-speech gestures [3, 7, 18, 42]. Initial deterministic models lacked expressiveness, leading to the adoption of generative methods that enable more synchronized, dynamic motion across regions [11, 15, 16, 24, 27]. For instance, Habibie et al. [41] proposed a CNN-based approach to jointly generate 3D facial and body keypoints, though it often failed to produce smooth coordination across body parts, leading to repetitive or disconnected gestures. TalkSHOW [1] advanced this by applying VQ-VAE with cross-conditioning to align body and hand gestures but treated facial expressions independently, resulting in fragmented expressions.
Other methods like DiffSHEG [2] and EMAGE [3], which use separate encoders for expressions and gestures to partially synchronize modalities through unidirectional flow, though this limits full expressive coherence. ProbTalk [4] uses PQ-VAE to better synchronize body and facial gestures, yet these methods often rely predominantly on rhythmic cues from audio, which, while effective for timing, may overshadow the importance of sparse, contextually meaningful semantic gestures that convey nuanced intent.

CHARM proposes a unified framework that integrates rhythmic consistency with semantic depth in co-speech gestures. Using a rhythmic consistency loss, CHARM enforces local and global rhythmic coherence across body regions, establishing a smooth base motion. Additionally, its semantic gating mechanism dynamically integrates frame-level semantic cues—such as text-based context and emotional tone—allowing CHARM to selectively generate gestures that align with both rhythmic flow and semantic meaning, enhancing naturalistic and contextually rich motion generation.

==> sec/3_method_script.tex <==
\section{Method}
\begin{figure}
    \centering
    \includegraphics[width=8cm]{overview.png}
    \caption{\textbf{An overview of the CHARM pipeline.} CHARM generates co-speech holistic  motion by first constructing rhythm-aligned  $q^{r}$ in \( f_r \), guided by rhythmic consistency loss \( L_{\text{Rhy}} \). Meanwhile, \( f_s \) produce frame-level semantic codes \( q^s \), activated selectively by the semantic score \( \psi \). Finally, \( q^m \) is achieved by fusing $q^{r}$ and \( q^s \) based on \( \psi \), with motion decoder, yielding synchronized and contextually enriched motions.}
    \label{fig:charm_overview}
\end{figure}

As illustrated in Figure \ref{fig:charm_overview}, our CHARM pipeline consists of two main components, i.e., the Base Motion Blocks \( f_r(\cdot) \) and the Sparse Motion Blocks \( f_s(\cdot) \). Given rhythmic features \( \gamma_b \), \( \gamma_h \), a seed pose \( \tilde{m} \), and a speaker ID \( id \), the Base Motion Blocks generate rhythm-aligned codes \( q^r \) to establish the motion’s rhythmic foundation, denoted as \( f_r \). This rhythm-aligned representation is optimized using the rhythmic consistency loss \( \mathcal{L}_{\text{Rhy}} \), enforcing temporal coherence with the audio rhythm. This process is formulated as:
\begin{equation}
f_r : (\gamma_b, \gamma_h, \tilde{m}, id; \theta_{f_r}) \rightarrow q^r,
\end{equation}
where \( \theta_{f_r} \) represents the learnable parameters of the Base Motion Blocks.
Subsequently, the Sparse Motion Blocks take semantic features \( \phi_l \), \( \phi_g \), and \( \phi_e \) along with \( \tilde{m} \) and \( id \) as inputs to produce frame-level semantic codes \( q^s \). The semantic score \( \psi \) selectively activates these codes to prioritize semantically significant frames, yielding a sparse motion representation \( f_s \). This process is formulated as:
\begin{equation}
f_s : (\phi_l, \phi_g, \phi_e, \tilde{m}, id; \theta_{f_s}) \rightarrow (q^s, \psi),
\end{equation}
where \( \theta_{f_s} \) represents the parameters of the Sparse Motion Blocks, and \( \psi \) serves as a gating mechanism that modulates \( q^s \) activation based on contextual relevance.
The semantic emphasis mechanism \(\mathcal{E}\) then combines the rhythm-aligned codes \( q^r \) and the semantic codes \( q^s \), guided by the semantic score \( \psi \), to form the final motion codes \( q^m \), which integrate both rhythmic and semantic information:
\begin{equation}
q^m = \mathcal{E}(q^r, q^s; \psi).
\end{equation}
Finally, the motion decoder takes \( q^m \) as input to generate the output motion \( m' \), enriched with both rhythm alignment and semantic emphasis:
Throughout this process, the rhythmic consistency loss \( \mathcal{L}_{\text{Rhy}} \), along with the seed pose \( \tilde{m} \) and speaker ID \( id \), ensures that the generated gestures maintain both rhythm alignment and frame level semantic relevance, achieving expressive, natural co-speech gestures.

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{methods3.png}
    \caption{\textbf{Architecture of CHARM.} CHARM generates co-speech holistic motion in three stages. (a) \textit{Base Motion Learning} uses rhythmic features \( \gamma_b \), \( \gamma_h \), seed pose \( \tilde{m} \), and \( id \) to produce rhythm-aligned codes \( q^r \) through \textit{Coarse2Fine Cross-Att Module} and guided by rhythmic consistency loss \( \mathcal{L}_{\text{Rhy}} \). (b) \textit{Sparse Motion Learning} fuses semantic features \( \phi_l \), \( \phi_g \), and \( \phi_e \) to generate semantic codes \( q^s \), activated by semantic score \( \psi \). (c) \textit{Adaptively Fusion} automatically combines \( q^r \) and \( q^s \) based on \( \psi \) to produce mixed codes \( q^m \) at frame level for contextually rich and rhythmically aligned motions.
 }
    \label{fig:method}
\end{figure*}

\subsection{Discrete Motion Prior Learning}
Our approach utilizes a residual vector-quantized autoencoder (RVQ-VAE) \cite{zeghidour2021soundstream,borsos2023audiolm,guo2024momask} to capture complex body movements with precision. Unlike standard VQ-VAE \cite{van2017neural}, which uses a single quantized latent space, RVQ-VAE allows us to decompose motion into multiple quantization levels, capturing both coarse and fine-grained details. To ensure that distinct body regions retain unique motion characteristics, we separate the body into three segments—upper body, hands, and lower body—assigning a specialized RVQ-VAE to each following \cite{ao2023gesturediffuclip,liu2024emage}. This segmentation allows us to encode the unique dynamics of each part while avoiding any undue entanglement of features across body areas.
Each body segment's motion sequence, denoted \( M = m_{1:N} \in \mathbb{R}^{N \times D} \), is mapped into a latent sequence \( z_{1:n} \in \mathbb{R}^{n \times d} \) using a 1D convolutional encoder with a downsampling factor of \( n/N \). This latent sequence enters the RVQ-VAE, which applies a series of quantization steps \( Q_1, Q_2, \ldots, Q_V \) to progressively encode fine details. Each quantization layer assigns the latent vector to the closest entry in its respective codebook, storing a residual difference at each step. This sequence of approximations captures nuanced movement across layers, ultimately producing a refined latent representation \( \hat{z} \), which is the cumulative sum of quantized codes from each layer. After that, the decoding process mirrors the encoding structure, with distinct decoders handling each body region independently.

\subsection{Generating Rhythm-related Base Motion}

The \textit{Base Motion Learning} in CHARM establishes a rhythmically aligned foundation for co-speech gesture generation by leveraging both rhythmic and speaker-specific features, enhancing the naturalness and personalization of generated gestures.

\textbf{Rhythmic Speech Encoding.} To synchronize motion with speech timing, CHARM incorporates rhythmic features beats \( \gamma_b \) and HuBERT features \( \gamma_h \). Beats \( \gamma_b \), derived from amplitude envelope, short-time energy, and onset detection, mark key rhythmic points for synchronizing gestures with the speech flow. Meanwhile, \( \gamma_h \), extracted through the HuBERT encoder \cite{hsu2021hubert}, captures high-level audio characteristics such as phonetic structure and speaker nuances, adding expressive detail to the gestures.

\textbf{Rhythm-Conditioned Motion Encoding.} Alongside rhythmic features, CHARM integrates an initial seed pose \( \tilde{m} \) and speaker identity \( id \) to produce a personalized, rhythm-aligned gesture foundation. The rhythmic features \( \gamma_b \) and \( \gamma_h \) are processed with the pose \( \tilde{m} \) and speaker ID \( id \) through a transformer-based block \textit{Corase2Fine Cross-Attn Module} to get latent base motion \( f_b\), later on with an MLP layer, generating codes that synchronize different body regions with the audio rhythm. This rhythm-conditioned encoding produces distinct codes for the face \( q^r_f \), hands \( q^r_h \), upper body \( q^r_u \), and lower body \( q^r_l \), ensuring temporal coherence across all components.

\textbf{Rhythmic Consistency Learning.} To enforce rhythmic alignment, we introduce a \textit{rhythmic consistency loss} \( \mathcal{L}_{\text{Rhy}} \), composed of two components: local frame-level InfoNCE loss \cite{chen2020simple} \( \mathcal{L}_{\text{Rhy}}^{(L)} \) and global sample-level InfoNCE loss \( \mathcal{L}_{\text{Rhy}}^{(G)} \). The local InfoNCE loss \( \mathcal{L}_{\text{Rhy}}^{(L)} \) aligns rhythm within each sample by maximizing the similarity between temporally aligned rhythmic features \( \gamma_h \) and latent face \( f_e \) and hand \( f_h \) features. This is defined as:
\begin{equation}
\mathcal{L}_{\text{Rhy}}^{(L)} = -\frac{1}{N} \sum_{i=1}^N \log \frac{\exp \left(\operatorname{sim}\left(h\left(f_i\right), g\left(\gamma_i\right)\right) / \tau \right)}{\sum_{j=1}^N \exp \left(\operatorname{sim}\left(h\left(f_i\right), g\left(\gamma_j\right)\right) / \tau \right)},
\end{equation}
where \( N \) is the number of frames, \(h(\cdot)\) and \(g(\cdot)\)are projection heads for the latent motion features and rhythmic features, respectively, \( f_i \) and \( \gamma_i \) represent the latent features \( (f_e, f_h) \) and rhythmic features at the \( i \)-th frame, respectively, \( \operatorname{sim}(\cdot) \) denotes cosine similarity, and \( \tau \) is the temperature hyperparameter. This loss encourages alignment between rhythmic features and frame-specific motion features, capturing meaningful temporal correlations. The global InfoNCE loss \( \mathcal{L}_{\text{Rhy}}^{(G)} \) reinforces rhythmic alignment across different samples by maximizing the similarity between \( \gamma_h \) and latent features \( (f_e, f_h) \) across sequences. By minimizing \(mathcal{L}_{Rhy}^{(L)}\) and \(mathcal{L}_{Rhy}^{(G)}\), the model learns to produce motion sequences that are both locally and globally consistent with the speech rhythm.

\textbf{Rhythmic Consistent Learning.} To reinforce rhythmic alignment across body regions, we introduce a dedicated learning objective, termed \textit{Rhythmic Consistent Learning}, designed to capture both local and global rhythm coherence in generated motions. This method employs a dual-level learning strategy through InfoNCE-based objectives: a local frame-level component, \( \mathcal{L}_{\text{Rhy}}^{(L)} \), and a global sample-level component, \( \mathcal{L}_{\text{Rhy}}^{(G)} \).

The local InfoNCE loss \( \mathcal{L}_{\text{Rhy}}^{(L)} \) aligns rhythm within each sample, encouraging the model to capture frame-specific correlations between rhythmic features \( \gamma_h \) and latent motion features (e.g., face \( f_e \) and hand \( f_h \) features). Defined as:
\begin{equation}
\mathcal{L}_{\text{Rhy}}^{(L)} = -\frac{1}{N} \sum_{i=1}^N \log \frac{\exp \left(\operatorname{sim}\left(h\left(f_i\right), g\left(\gamma_i\right)\right) / \tau \right)}{\sum_{j=1}^N \exp \left(\operatorname{sim}\left(h\left(f_i\right), g\left(\gamma_j\right)\right) / \tau \right)},
\end{equation}
where \( N \) is the number of frames, \( h(\cdot) \) and \( g(\cdot) \) are projection heads for latent motion features and rhythmic features, respectively, \( f_i \) and \( \gamma_i \) represent latent and rhythmic features at frame \( i \), and \( \operatorname{sim}(\cdot) \) denotes cosine similarity. This loss encourages the alignment of motion features with rhythm on a frame-by-frame basis, ensuring that the generated motion reflects subtle rhythmic variations.

The global InfoNCE loss \( \mathcal{L}_{\text{Rhy}}^{(G)} \), on the other hand, reinforces rhythmic coherence across sequences by maximizing the similarity between global rhythmic features \( \gamma_h \) and latent motion features (e.g., \( f_e \) and \( f_h \)) across different samples. By optimizing both \( \mathcal{L}_{\text{Rhy}}^{(L)} \) and \( \mathcal{L}_{\text{Rhy}}^{(G)} \), our model learns to generate motion sequences that are rhythmically consistent both within individual frames and across entire sequences, establishing a solid, rhythm-aligned foundation for further semantic enhancement.

Through this two-tiered approach in Rhythmic Consistent Learning, CHARM produces base motions that are rhythmically coherent and finely tuned to the timing and flow of speech, setting the stage for seamless integration with sparse, semantically relevant gestures.

\subsection{Generating Semantic-aware Sparse Motion}  


The \textit{Sparse Motion Learning} in CHARM augments the rhythm-aligned base motion with expressive, contextually nuanced gestures by selectively integrating semantically meaningful information derived from speech content and emotional tone. This stage achieves semantic enhancement through three core components: a Semantic Speech Encoding module, a Semantic Gating Mechanism, and a hierarchical Coarse-to-Fine Body-Part Refinement.

\textbf{Semantic Speech Encoding.} To capture the full semantic spectrum of speech, the Sparse Motion Learning fuses three levels of information: frame-level text embeddings \( \phi_l \), sentence-level features \( \phi_g \) from the CLIP model \cite{radford2021learning}, and emotion features \( \phi_e \) derived from the emotion2vec model \cite{ma2023emotion2vec}. These features, which encompass both local and global contexts, are combined to form a comprehensive semantic representation \( f_t \). This representation not only reflects the textual elements of the spoken content but also captures emotional undertones, allowing CHARM to enhance gestures by activating expressive elements that align with nuanced speech cues.

\textbf{Semantic Gating Mechanism.} The fused semantic representation \( f_t \) is processed through a \textit{Semantic Gate} to compute frame-specific semantic scores \( \psi \), which selectively activate gestures at frames where semantic relevance is high. By focusing on high-relevance frames, this gating mechanism ensures that the network’s attention aligns with sparse semantic gestures, retaining the underlying rhythmic structure while injecting contextual emphasis where needed. The Semantic Gate, informed by both local and global semantics within \( f_t \), applies the semantic score \( \psi \) to modulate the latent base motion \( f_b \) and the sparse motion \( f_s \) through alpha-blending. It's optional that the frame-specific semantic labels from the dataset can further supervise \( \psi \) as \(\mathcal{L}^G_{cls}\), ensuring accurate alignment with the intended speech content.

\textbf{Coarse-to-Fine Body-Part Refinement.} The gated semantic features, represented by \( f_t \), flow into a hierarchical \textit{Coarse2Fine Cross-Attention Module}, which refines the semantic representation for each body part. This hierarchical structure begins by generating face-specific features \( f_e^s \) and proceeds to condition the hands, upper body, and lower body in sequence. Specifically, \( f_e^s \) serves as the base for hand features \( f_h^s \), which in turn guide the upper body features \( f_u^s \), and together, these features inform the lower body representation \( f_l^s \). Each refinement stage leverages cross-attention to align the rhythmic and semantic aspects across the body, resulting in coherent and contextually relevant gestures. Note that the flow \( f_e^s \) guide \( f_h^s \) only happens in \textit{Base Motion Learning}, in this stage, the model doesn't generate codes of face, since the sparse motion mainly focuses on the body part.

To produce the final output codes, \( q^s \), the alpha-blended combination of \( f_b \) and \( f_s \), weighted by the semantic score \( \psi \), is processed through a multilayer perceptron (MLP) to obtain the final motion codes. This combination is defined as:
\[
q^s = MLP(\psi f_s + (1 - \psi) f_b),
\]
where \( q^s \) reflects frames with high semantic importance by drawing more from \( f_s \), while less relevant frames rely predominantly on \( f_b \). 

To promote diversity in the generated gestures, both the latent code classification cross-entropy loss \( \mathcal{L}^{R}_{cls} \) and the latent reconstruction loss \( \mathcal{L}^{R}_{rec} \) are optimized. Additionally, a threshold \( \beta \) is applied to \( \psi \) to retain the loss of frames above this threshold, emphasizing sparse, semantically-rich gestures not learned by the Base Motion Learning. This dual-loss approach encourages CHARM to generate a range of gestures that align with varied semantic cues, enhancing the overall output's expressiveness and context sensitivity.


\subsection{Coherent and Expressive Motion Generator}

The \textit{Semantic Emphasis Stage} in CHARM is designed to seamlessly integrate sparse, contextually rich gestures into the rhythmically aligned base motion. This stage selectively enhances prominent gestures based on their semantic importance, while maintaining a smooth, natural motion flow across frames.

\textbf{Adaptive Code Replacement.} In this stage, CHARM dynamically chooses which frames to emphasize based on the semantic scores calculated in the previous \textit{Sparse Motion Learning}. For each frame \( i \), the semantic score \( \psi_i \) is compared against a threshold \( \beta \) to identify frames with significant semantic relevance. When \( \psi_i > \beta \), the latent code \( q_i^r \) in the base motion is replaced by the sparse semantic code \( q_i^s \), effectively highlighting frames where expressive, meaningful gestures are most relevant:
\[
q_i = \begin{cases} 
      q_i^s & \text{if } \psi_i > \beta, \\
      q_i^r & \text{otherwise}.
   \end{cases}
\]
This selective replacement ensures that semantically critical gestures receive enhanced emphasis, without disrupting the natural rhythmic flow of the overall motion.

\textbf{Semantic Blending and Natural Flow Preservation.} By selectively blending \( q^r \) and \( q^s \) based on semantic scores, CHARM maintains continuity between emphasized gestures and the underlying rhythm. This integration not only preserves the coherence of the motion but also adapts to the expressive needs of the speech context. The result is a fluid motion sequence where important gestures stand out without breaking the foundational rhythm. To ensure harmonious transitions, we apply this replacement operation on a frame-by-frame basis across all body parts. This approach maintains frame-level consistency, avoiding abrupt shifts while emphasizing expressive frames.


\subsection{Generating Rhythm-related Base Motion}

The \textit{Rhythmic Consistent Learning} in CHARM establishes a rhythmically aligned foundation for generating co-speech gestures by learning general rhythm-related motion patterns that synchronize seamlessly with the audio rhythm.

\textbf{Rhythmic Speech Encoding.} To align gesture timing with speech, CHARM utilizes rhythmic features, including beats \( \gamma_b \) and high-level audio features \( \gamma_h \) from HuBERT \cite{hsu2021hubert}. Beats \( \gamma_b \) mark key rhythmic points, while \( \gamma_h \) captures nuanced phonetic and speaker-specific details, adding expressiveness to the generated gestures. These features, combined with an initial pose \( \tilde{m} \) and speaker ID \( id \), pass through a \textit{Coarse2Fine Cross-Attention Module} and MLP to produce synchronized base motion representations \( f_b \), which encode rhythm-aligned codes for the face \( q^r_f \), hands \( q^r_h \), upper body \( q^r_u \), and lower body \( q^r_l \), establishing coherence across all body regions.

\textbf{Rhythmic Consistent Learning.} To enforce a rhythmically coherent base motion, we introduce \textit{Rhythmic Consistent Learning}, which includes both local and global consistency components designed to align generated gestures with the natural timing of speech. While inspired by CoG’s \cite{xu2024chain} use of InfoNCE loss \cite{chen2020simple} for synchronizing facial expressions with audio cues, our approach differs fundamentally by applying separate local and global rhythmic consistency losses across both gestures and facial features. This multi-dimensional alignment ensures that each body region maintains synchronized rhythm with the audio, creating a cohesive foundation for co-speech motion.

The local frame-level consistency loss \( \mathcal{L}_{\text{Rhy}}^{(L)} \) aligns each frame's motion features with the corresponding rhythmic cues, maximizing temporal coherence between rhythmic features \( \gamma_h \) and the latent motion features for the face \( f_e \) and hands \( f_h \). This is defined as:
\begin{equation}
\mathcal{L}_{\text{Rhy}}^{(L)} = -\frac{1}{N} \sum_{i=1}^N \log \frac{\exp \left(\operatorname{sim}\left(h\left(f_i\right), g\left(\gamma_i\right)\right) / \tau \right)}{\sum_{j=1}^N \exp \left(\operatorname{sim}\left(h\left(f_i\right), g\left(\gamma_j\right)\right) / \tau \right)},
\end{equation}
where \( N \) denotes the number of frames, \( h(\cdot) \) and \( g(\cdot) \) are projection heads for latent motion and rhythmic features, \( f_i \) and \( \gamma_i \) are the latent and rhythmic features at frame \( i \), and \( \operatorname{sim}(\cdot) \) represents cosine similarity. This local loss encourages each frame's gestures and facial movements to align with subtle rhythmic variations, embedding rhythm within each temporal segment.

To ensure rhythmic coherence at a broader level, we incorporate a global sample-level consistency loss \( \mathcal{L}_{\text{Rhy}}^{(G)} \), which reinforces alignment across the entire motion sequence. This global loss is defined as:
\begin{equation}
\mathcal{L}_{\text{Rhy}}^{(G)} = - \log \frac{\exp \left( \operatorname{sim} \left( H(f), G(\gamma) \right) / \tau \right)}{\sum_{k} \exp \left( \operatorname{sim} \left( H(f), G(\gamma^{(k)}) \right) / \tau \right)},
\end{equation}
where \( H(f) \) and \( G(\gamma) \) denote the global embeddings of the entire latent motion features and rhythmic features, respectively, and \( \gamma^{(k)} \) represents the rhythmic features from other samples in the batch. This global loss encourages rhythm consistency over the entire sequence, ensuring that the generated motion maintains a coherent flow aligned with the speech rhythm across the duration of the sequence.

By jointly minimizing \( \mathcal{L}_{\text{Rhy}}^{(L)} \) and \( \mathcal{L}_{\text{Rhy}}^{(G)} \), Rhythmic Consistent Learning enables CHARM to produce base motions that are both rhythmically aligned and temporally cohesive, forming a solid foundation upon which further semantic gesture refinement can be applied.

\subsection{Generating Semantic-aware Sparse Motion}

The \textit{Semantic Emphasis Learning} in CHARM adds expressive, context-specific gestures to the rhythm-aligned base motion by incorporating sparse but meaningful semantic cues drawn from speech content and emotional tone. By separating rhythm and semantics, this stage enhances gesture generation with contextually nuanced movements, focusing on moments of high semantic relevance.

\textbf{Semantic Speech Encoding.} To capture the breadth of semantic cues in speech, Semantic Emphasis Learning combines three types of information: frame-level text embeddings \( \phi_l \), sentence-level features \( \phi_g \) from the CLIP model \cite{radford2021learning}, and emotion features \( \phi_e \) from the emotion2vec model \cite{ma2023emotion2vec}. Together, these features form a comprehensive semantic representation \( f_t \) that reflects both the content and emotional undertones of speech, enabling CHARM to activate gestures that are sensitive to nuanced semantic cues.

\textbf{Semantic Emphasis Learning.} \textit{Semantic Emphasis Learning} is designed to capture sparse, semantically rich gestures that complement the rhythmically consistent base motion, allowing CHARM to selectively enhance gestures at moments of high semantic relevance. This approach focuses on infrequent yet impactful gestures that convey specific meanings or emotions, adding depth and expressiveness to co-speech motion.

To determine which frames require additional emphasis, we leverage a fused semantic representation \( f_t \). This multi-level fusion allows the model to recognize frames where gestures should convey heightened meaning. A learned semantic score \( \psi \), derived from \( f_t \), dynamically adjusts the integration of rhythm-aligned base motion \( f_b \) and sparse semantic motion \( f_s \). For frames with high semantic scores, the model emphasizes \( f_s \), while frames with lower relevance continue to rely on \( f_b \). This selective enhancement ensures that semantically significant gestures are dynamically incorporated without disrupting the underlying rhythmic flow.

In refining the semantic emphasis across body regions, CHARM employs a \textit{Coarse2Fine Cross-Attention Module} that hierarchically conditions the semantic features from the face to the hands, then to the upper body, and finally to the lower body. Beginning with the face, the model generates semantic features \( f_e^s \) that influence the hand features \( f_h^s \), which in turn guide the upper body \( f_u^s \) and lower body \( f_l^s \). This hierarchical conditioning ensures that the semantic emphasis flows naturally through each body part, enabling coherent and contextually relevant gestures that align with spoken content. In this stage, the focus is on body gestures rather than facial expressions, as body movements are critical for expressing semantic meaning in speech-driven gestures.

The final motion codes \( q^s \) are produced by blending \( f_b \) and \( f_s \) based on the semantic score \( \psi \) and refining this blend through an MLP, defined as:
\[
q^s = MLP(\psi f_s + (1 - \psi) f_b),
\]
where frames with higher semantic scores rely more on \( f_s \), and less relevant frames maintain the rhythm-aligned base \( f_b \). This blending approach allows the model to produce gestures that are not only rhythmically consistent but also carry semantic weight in key frames.

To support the generation of diverse gestures, we incorporate a dual-loss framework with a latent code classification loss \( \mathcal{L}^{R}_{cls} \) and a reconstruction loss \( \mathcal{L}^{R}_{rec} \). Additionally, a threshold \( \beta \) is applied to \( \psi \) to retain losses for frames with high semantic scores, further encouraging the model to focus on sparse, contextually significant gestures that augment the rhythm-based base motion. This approach allows CHARM to produce gestures that are both expressive and responsive to the subtleties of speech, effectively balancing rhythm with semantic depth.

\textbf{Semantic Emphasis Learning.} In the \textit{Semantic Emphasis Learning} stage, CHARM selectively enhances sparse, semantically rich gestures by identifying frames that carry significant meaning within the context of speech. This approach complements the rhythm-aligned base motion by focusing on expressive movements at critical points, capturing the depth of communication in co-speech gestures.

The process begins by using fused semantic features \( f_t \), which contain both local and global levels of information from text, speech, and emotion embeddings. This comprehensive representation enables the model to capture context at multiple levels, allowing it to respond to the nuanced needs of each frame. The semantic score \( \psi \), derived from this feature mix, is used to assess the relevance of each frame. By leveraging global context within \( f_t \), \( \psi \) can learn to emphasize frames with high semantic importance while ignoring those that contribute only to the general rhythmic flow.

Once calculated, the semantic score \( \psi \) modulates the combined semantic features \( f_t \) by re-weighting them based on relevance, effectively filtering out frames with low semantic value and ensuring the network’s attention is focused on frames that align with specific communicative intentions. This targeted emphasis allows the network to activate only those frames that carry sparse, high-relevance gestures, adding a layer of semantic richness to the base rhythm.

To incorporate the semantic emphasis into the generated motion, the score \( \psi \) is further supervised by a classification loss \( \mathcal{L}_{cls}^{G} \), which is aligned with semantic frame labels in the dataset, ensuring that \( \psi \) accurately identifies and reinforces frames that convey distinct meaning. The score \( \psi \) then alpha-blends the latent base motion \( f_b \) with the latent sparse motion \( f_s \), effectively integrating rhythm and semantics. This blending process creates the final motion codes \( q^s \) through an MLP layer:
\[
q^s = MLP(\psi f_s + (1 - \psi) f_b),
\]
where frames with high semantic scores draw more from \( f_s \), while less relevant frames remain grounded in the rhythm-aligned base \( f_b \).

To encourage the diversity and expressiveness of generated gestures, we incorporate a dual-loss structure composed of a latent code classification loss \( \mathcal{L}^{R}_{cls} \) and a reconstruction loss \( \mathcal{L}^{R}_{rec} \). Additionally, by applying a threshold \( \beta \) to \( \psi \), we retain losses only for frames where semantic scores surpass this threshold, guiding the model toward emphasizing sparse, contextually rich gestures.




































==> sec/table_fig.tex <==
% \begin{table*}[t]
%    \centering
%     \setlength{\tabcolsep}{4pt} % 调整列间距
%     \resizebox{0.8\textwidth}{!}{\begin{tabular}{llccccc llccccc}
%         \toprule
%         \multicolumn{6}{c}{\textbf{BEAT2 Dataset}} & \multicolumn{6}{c}{\textbf{SHOW Dataset}} \\
%         \textbf{Method} & \textbf{FGD$\downarrow$} & \textbf{BC$\uparrow$} & \textbf{DIV$\uparrow$} & \textbf{MSE$\downarrow$} & \textbf{LVD$\downarrow$} &
%         & \textbf{Method} & \textbf{FGD$\downarrow$} & \textbf{BC$\uparrow$} & \textbf{DIV$\uparrow$} & \textbf{MSE$\downarrow$} & \textbf{LVD$\downarrow$} \\
%         \midrule
%         FaceFormer~\cite{fan2022faceformer} & - & - & - & 7.787 & 7.593 & & FaceFormer~\cite{fan2022faceformer} & - & - & - & 137.7 & 43.86 \\
%         CodeTalker~\cite{xing2023codetalker} & - & - & - & 8.026 & 7.766 & & CodeTalker~\cite{xing2023codetalker} & - & - & - & 140.2 & 45.54 \\
%         CaMN~\cite{liu2022beat} & 6.644 & 6.769 & 10.86 & - & - & & CaMN~\cite{liu2022beat} & 2.199 & 7.998 & 10.13 & - & - \\
%         DSG~\cite{yang2023diffusestylegesture} & 8.811 & 7.241 & 11.49 & - & - & & DSG~\cite{ref37} & 2.404 & 8.295 & 10.04 & - & - \\
%         Habibie \textit{et al.}~\cite{habibie2021learning} & 9.040 & 7.716 & 8.213 & 8.614 & 8.043 & & Habibie \textit{et al.}~\cite{habibie2021learning} & 2.679 & 8.510 & 8.055 & 145.1 & 47.11 \\
%         TalkSHOW~\cite{yi2023generating} & 6.209 & 6.947 & \textbf{13.47} & 7.791 & 7.771 & & TalkSHOW~\cite{yi2023generating} & 2.462 & 8.449 & 10.29 & 139.3 & 44.81 \\
%         EMAGE~\cite{liu2024emage} & 5.512 & 7.724 & 13.06 & 7.680 & 7.556 & & EMAGE~\cite{liu2024emage} & 2.255 & 8.585 & \textbf{12.40} & 136.4 & 42.74 \\
%         DiffSHEG~\cite{chen2024diffsheg} & 12.70 & 7.142 & 11.91 & 7.665 & 8.673 & & DiffSHEG~\cite{chen2024diffsheg} & 2.417 & 8.461 & 12.29 & 13 & 8.673 \\
%         \cmidrule(lr){1-6} \cmidrule(lr){8-13}
%         \textbf{CHARM (Ours)} & \textbf{4.178} & \textbf{7.724} & 13.21 & \textbf{6.100} & \textbf{6.938} & & \textbf{CHARM (Ours)} & \textbf{4.178} & \textbf{7.724} & 13.21 & \textbf{6.100} & \textbf{6.938} \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Quantitative comparison with SOTA methods on the SHOW and BEAT2 datasets. Lower values are better for FMD, FGD, MSE, and LVD. Higher values are better for BC and DIV.}
%     \label{tab:show_beat2_comparison}
% \end{table*}
